A level line of the Gaussian free field with measure-valued boundary conditions

In this article, we construct samples of SLE-like curves out of samples of CLE and Poisson point process of Brownian excursions. We show that the law of these curves depends continuously on the intensity measure of the Brownian excursions. Using such construction of curves, we extend the notion of level lines of GFF to the case when the boundary condition is measure-valued.

==> tex202102/macro_hao.tex <==

%%%%%%%%mathcal%%%%%%%
\newcommand{\LA}{\mathcal{A}}
\newcommand{\LB}{\mathcal{B}}
\newcommand{\LC}{\mathcal{C}}
\newcommand{\LD}{\mathcal{D}}
\newcommand{\LE}{\mathcal{E}}
\newcommand{\LF}{\mathcal{F}}
\newcommand{\LG}{\mathcal{G}}
\newcommand{\LH}{\mathcal{H}}
\newcommand{\LI}{\mathcal{I}}
\newcommand{\LJ}{\mathcal{J}}
\newcommand{\LK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\LM}{\mathcal{M}}
\newcommand{\LN}{\mathcal{N}}
\newcommand{\LO}{\mathcal{O}}
\newcommand{\LP}{\mathcal{P}}
\newcommand{\LQ}{\mathcal{Q}}
\newcommand{\LR}{\mathcal{R}}
\newcommand{\LS}{\mathcal{S}}
\newcommand{\LT}{\mathcal{T}}
\newcommand{\LU}{\mathcal{U}}
\newcommand{\LV}{\mathcal{V}}
\newcommand{\LW}{\mathcal{W}}
\newcommand{\LX}{\mathcal{X}}
\newcommand{\LY}{\mathcal{Y}}
\newcommand{\LZ}{\mathcal{Z}}


